Optimal transport on gas networks

This paper models gas networks as metric graphs, with isothermal Euler equations at the edges, Kirchhoff's law at interior vertices and time-(in)dependent boundary conditions at boundary vertices. For this setup, a generalized $p$-Wasserstein metric in a dynamic formulation is introduced and utilized to derive $p$-Wasserstein gradient flows, specifically focusing on the non-standard case $p = 3$.

==> 5.1_curves_velocity_fields.tex <==
\subsection{$p$-absolutely continuous curves and velocity fields}

\noindent As we are interested in the graph setting, we will set $\Omega := \Omega_{\mathcal{G}}$ and $d := W_p$ \af{OR} $d := \left\lvert x - y\right\rvert$. \af{TODO double integration over time ???}

\begin{theorem}[Connection $p$-absolutely continuous curves and velocity fields] ~ \\
    Let
    \begin{equation*}
        \mu: \left(0, T\right) \longrightarrow \Omega_{\mathcal{G}} \quad t \mapsto \mu\left(t\right)
    \end{equation*}
    be a curve and 
    \begin{equation*}
        V: \Omega_{\mathcal{G}} \times \left(0, T\right) \longrightarrow \mathbb{R}^{d + 1} \quad \left(x, t\right) \mapsto V\left(x, t\right) ~ \text{\af{TODO correct dimension???}}
    \end{equation*}
    a vector field, then the following two statements hold true:
    \begin{itemize}
        \item[1)] $\mu \in AC^p \left(0, T, \Omega_{\mathcal{G}}\right) \quad \Longrightarrow \quad$ for a.e. $t \in \left(0, T\right): \, \exists V \in L^p\left(\mu\right): \, ||V||_{L^p\left(\mu\right)} \leq \left\lvert \mu' \left(t\right) \right\rvert$ and $\left(\mu, \mu V\right)$ is a weak solution
        \item[2)] $\left(\mu, \mu V\right)$ is a weak solution with $\int_0^T ||v||_{L^p\left(\mu\right)} \, \mathrm d t < \infty \quad \Longrightarrow \quad \mu \in AC^p \left(0, T, \Omega_{\mathcal{G}}\right)$ and for a.e. $t \in \left(0, T\right): \, \left\lvert \mu' \left(t\right) \right\rvert \leq ||v||_{L^p\left(\mu\right)}$
    \end{itemize}
\end{theorem}

==> 5_OT_minimizers.tex <==
\section{Existence of minimizers for the dynamical optimal transport task} \label{sec:existence}

Before presenting the main results of this section, we need to introduce some further concepts and notations. \af{NOT EDITED YET}\\

\begin{definition}[$p$-absolutely continuous curves \cite{ambrosio2005gradient}, \cite{erbar2021gradient}] ~ \\
    For a complete metric space $\left(\mathcal{X}, d\right)$ with $\Omega \subseteq \mathbb{R}^d$, we call a curve
    \begin{equation*}
        \mu: \left(0, T\right) \longrightarrow \mathcal{X} \quad t \mapsto \mu\left(t\right),
    \end{equation*}
    $p$-absolutely continuous for $p \in \left[1, \infty\right)$, if there exists a function $g \in L^p \left(\left(0, T\right), \left(\mathbb{R}, \left\lvert \, \cdot \, \right\rvert\right), \eta\right)$ such that
    \begin{equation}
        \label{abscont}
        \forall 0 < r \leq s < T: \, d \left(\mu \left(r\right), \mu \left(s\right)\right) \leq \int_r^s g \left(t\right) \, \mathrm d t
    \end{equation}
    where $L^p \left(\left(\left(0, T\right), \eta\right), \left(\mathbb{R}, \left\lvert \, \cdot \, \right\rvert\right)\right)$ denotes the $L^p$-space of $\eta$-measurable and $\mathbb{R}$-valued functions on the interval $\left(0, T\right)$, so
    \begin{equation*}
        L^p \left(\left(\left(0, T\right), \eta\right), \left(\mathbb{R}, \left\lvert \, \cdot \, \right\rvert\right)\right) := 
    \end{equation*}
    \begin{equation*}
        \left\{g: \left(0, T\right) \longrightarrow \mathbb{R} \quad \eta-\text{measurable} ~ \middle| ~ \int_0^T \left\lvert g\left(t\right) - \tilde{x} \right\rvert^p \, \mathrm d \eta\left(t\right) < \infty ~ \text{for some} ~ \tilde{x} \in \mathbb{R}\right\}
    \end{equation*}
    (with the finiteness of the integral not depending on the choice of $\tilde{x}$), and where we choose the one-dimensional Lebesgue measure $\mathcal{L}$ on $\left[0, T\right]$ as $\eta$, thus for $X \subseteq \left[0, T\right]$ we obtain
    \begin{equation*}
        \eta \left(X\right) = \mathcal{L} \left(X\right) = 
    \end{equation*}
    \begin{equation*}
        \inf \left\{\sum_{k = 1}^{\infty} \left(b_k - a_k\right) ~ \middle|
        \begin{array}{l}
            \left(a_k, b_k\right)_{k \in \mathbb{N}} ~ \text{sequence of open intervals with} ~ a_k, b_k \in \mathbb{R}, \vspace{0.1cm} \\
            a_k \leq b_k ~ \text{and} ~ X \subseteq \bigcup_{k = 1}^{\infty} \left(a_k, b_k\right)
        \end{array}\right\}. 
    \end{equation*}

    \noindent By $AC^p \left(\left(0, T\right), \mathcal{X}, \eta\right)$ we will denote the corresponding space of $p$-absolutely continuous curves on the complete metric space $\left(\mathcal{X}, d\right)$ with respect to the measure $\eta$. \\
\end{definition}

\noindent Among all possible function choices of $g$ in (\ref{abscont}), we are interested in the minimal one, whose existence is given by the following proposition. \\

\begin{proposition}[Metric derivative of $p$-absolutely continuous curves \cite{ambrosio2005gradient}] ~ \\
    For every $p$-absolutely continuous curve $\mu \in AC^p \left(\left(0, T\right), \mathcal{X}, \mathcal{L}\right)$, the limit
    \begin{equation*}
        \left\lvert \mu' \left(t\right) \right\rvert := \lim_{r \rightarrow s} \frac{d\left(\mu\left(r\right), \mu\left(s\right)\right)}{\left\lvert r - s \right\rvert}
    \end{equation*}
    exists for $\mathcal{L}$-a.e. $s \in \left(0, T\right)$ and the function $t \mapsto \left\lvert \mu' \left(t\right) \right\rvert$ belongs to $L^p \left(\left(0, T\right), \mathbb{R}, \mathcal{L}\right)$. Furthermore, $\left\lvert \mu' \left(t\right) \right\rvert$ is an admissible choice for $g$ and minimal in the sense of
    \begin{equation*}
        \left\lvert \mu' \left(t\right) \right\rvert \leq \tilde{g}\left(t\right) ~ \text{for} ~ \mathcal{L} \text{-a.e.} ~ t \in \left(0, T\right)
    \end{equation*}
    for each function $\tilde{g} \in L^p \left(\left(0, T\right), \mathbb{R}, \mathcal{L}\right)$ satisfying (\ref{abscont}).
\end{proposition}

\begin{proof}
    See for example Theorem 1.1.2 in \cite{ambrosio2005gradient}.
\end{proof}

==> scraps.tex <==
This subset of vertices is given by
\begin{equation*}
    \mathcal{V}_{\geq 2} := \left\{\nu \in \mathcal{V} ~ \middle| ~ \deg \left(\nu\right) \geq 2\right\},
\end{equation*}
where we define the vertex degree function as
\begin{equation*}
    \deg: \mathcal{V} \longrightarrow \mathbb{N}_{\geq 0} \quad \nu \mapsto \deg \left(\nu\right) := \left\lvert \left\{e \in \mathcal{E} ~ \middle| ~ \nu \in e\right\}\right\rvert,
\end{equation*}
which returns for each vertex $\nu \in \mathcal{V}$ the number of incident edges $e \in \mathcal{E}$ in the graph. Note that, isolated vertices (vertices which are not connected to any other vertex) have degree $0$ and vertices at the boundary of the network have degree $1$. Since we want to consider vertices modelling the intersection of at least two pipes, we are only interested in vertices with a degree of at least $2$.\\





\noindent Before presenting the definition of weak solutions, we want to give a brief introduction into the underlying reformulations. The detailed calculations can be found in the appendix. \\

\begin{observation}[Derivation of weak solutions] ~ \\
    Suppose $\left(\rho, j\right)$ to be a strong solution of (\ref{eqn:OT C KL}) without any boundary vertices, and let
    \begin{equation*}
        \varphi : \Omega_{\mathcal{G}} \times \left[0, T\right] \longrightarrow \mathbb{R} \quad \left(x, t\right) \mapsto \varphi \left(x, t\right)
    \end{equation*}
    be a continuously differentiable \textbf{test function}, then for the test function at vertex $\nu \in \mathcal{V}$ at time $t \in \left[0, T\right]$ we write $\varphi_{\nu} \left(t\right)$, and similarly at $x \in \left[0, L_e\right]$ for any edge $e \in \mathcal{E}$ at time $t \in \left[0, T\right]$ we write $\varphi_e \left(x, t\right)$. \\

    \noindent Integration by parts of the continuity equation at any edge $e \in \mathcal{E}$ multiplied by the test function $\varphi$ yields
    \begin{equation*}
        0 = \int_0^{L_e} \frac{\partial \rho_e}{\partial t} \varphi_e \, \mathrm d x + \Big[j_e \varphi_e\Big]_0^{L_e} - \int_0^{L_e} j_e \frac{\partial \varphi_e}{\partial x} \, \mathrm d x . \\
    \end{equation*}

    \noindent Moreover, summing over all edges $e \in \mathcal{E}$ and utilizing Kirchhoff's law as well as the continuity of the test function results in:
    \begin{flalign*}
        \sum_{e \in \mathcal{E}} \int_0^{L_e} \frac{\partial j_e}{\partial x} \varphi_e \, \mathrm d x & = \sum_{e \in \mathcal{E}} \int_0^{L_e} \frac{\partial \rho_e}{\partial t} \varphi_e \, \mathrm d x + \sum_{\nu \in \mathcal{V}} \left( \sum_{\substack{e \in \mathcal{E}: \\ \delta^E \left(e\right) = \nu}} \left. j_e \right|_{x = \nu} - \sum_{\substack{e \in \mathcal{E}: \\ \delta^S \left(e\right) = \nu}} \left. j_e \right|_{x = \nu}\right) \varphi_{\nu} \\
        & = \sum_{e \in \mathcal{E}} \int_0^{L_e} \frac{\partial \rho_e}{\partial t} \varphi_e \, \mathrm d x
    \end{flalign*}
\end{observation}
